Blockchain Transaction Conflicts: A Historical Perspective

This paper presents a comprehensive analysis of historical data across two popular blockchain networks: Ethereum and Solana. Our study focuses on two key aspects: transaction conflicts and the maximum theoretical parallelism within historical blocks. We aim to quantify the degree of transaction parallelism and assess how effectively it can be exploited by systematically examining block-level characteristics, both within individual blocks and across different historical periods. In particular, this study is the first of its kind to leverage historical transactional workloads to evaluate conflict patterns. By offering a structured approach to analyzing these conflicts, our research provides valuable insights and an empirical basis for developing more efficient parallel execution techniques for smart contracts in the Ethereum and Solana. Our empirical analysis reveals that historical Ethereum blocks frequently achieve high independence, with over 50\% independent transactions in more than 50\% of blocks, while, on average, Solana blocks contain longer conflict chains $\sim$58\%, compared to $\sim$18\% in Ethereum, reflecting fundamentally different parallel execution dynamics.

==> figs/access_vs_rwset.tex <==
\begin{tikzpicture}[scale = .85, x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,166); %set diagram left start at 0, and has height of 166

%Straight Lines [id:da27291330854129225] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }]   (49.08,28.96) -- (49.08,49.13) ;
%Straight Lines [id:da8480208573951736] 
\draw [color={rgb, 255:red, 14; green, 20; blue, 233 }]   (247.17,78.96) -- (247.17,99.13) ;
%Straight Lines [id:da6681878623568541] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }]   (239.17,28.79) -- (239.17,48.96) ;
%Straight Lines [id:da7109562684347461] 
\draw [color={rgb, 255:red, 14; green, 20; blue, 233 }]   (457.17,79.21) -- (457.17,99.38) ;
%Straight Lines [id:da03546319242071849] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }]   (49.08,39.04) -- (239.17,38.88) ;
%Straight Lines [id:da9482342600998073] 
\draw [color={rgb, 255:red, 14; green, 20; blue, 233 }]   (247.17,89.04) -- (457.17,89.29) ;
%Shape: Circle [id:dp6248910885677119] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }][fill={rgb, 255:red, 128; green, 128; blue, 128 }] (76.14,39.21) .. controls (76.14,37.32) and (77.68,35.79) .. (79.57,35.79) .. controls (81.46,35.79) and (83,37.32) .. (83,39.21) .. controls (83,41.11) and (81.46,42.64) .. (79.57,42.64) .. controls (77.68,42.64) and (76.14,41.11) .. (76.14,39.21) -- cycle ;
%Shape: Circle [id:dp9902796793524257] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }][fill={rgb, 255:red, 128; green, 128; blue, 128 }] (195.14,38.71) .. controls (195.14,36.82) and (196.68,35.29) .. (198.57,35.29) .. controls (200.46,35.29) and (202,36.82) .. (202,38.71) .. controls (202,40.61) and (200.46,42.14) .. (198.57,42.14) .. controls (196.68,42.14) and (195.14,40.61) .. (195.14,38.71) -- cycle ;
%Shape: Circle [id:dp2831853603872543] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }][fill={rgb, 255:red, 128; green, 128; blue, 128 }] (579.14,38.71) .. controls (579.14,36.82) and (580.68,35.29) .. (582.57,35.29) .. controls (584.46,35.29) and (586,36.82) .. (586,38.71) .. controls (586,40.61) and (584.46,42.14) .. (582.57,42.14) .. controls (580.68,42.14) and (579.14,40.61) .. (579.14,38.71) -- cycle ;
%Shape: Circle [id:dp11547972450766453] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }][fill={rgb, 255:red, 128; green, 128; blue, 128 }] (703.64,38.71) .. controls (703.64,36.82) and (705.18,35.29) .. (707.07,35.29) .. controls (708.96,35.29) and (710.5,36.82) .. (710.5,38.71) .. controls (710.5,40.61) and (708.96,42.14) .. (707.07,42.14) .. controls (705.18,42.14) and (703.64,40.61) .. (703.64,38.71) -- cycle ;
%Shape: Circle [id:dp3041445043459807] 
\draw  [color={rgb, 255:red, 14; green, 20; blue, 233 }][fill={rgb, 255:red, 14; green, 20; blue, 233 }] (596.64,88.71) .. controls (596.64,86.82) and (598.18,85.29) .. (600.07,85.29) .. controls (601.96,85.29) and (603.5,86.82) .. (603.5,88.71) .. controls (603.5,90.61) and (601.96,92.14) .. (600.07,92.14) .. controls (598.18,92.14) and (596.64,90.61) .. (596.64,88.71) -- cycle ;
%Shape: Circle [id:dp778012637561726] 
\draw  [color={rgb, 255:red, 14; green, 20; blue, 233 }][fill={rgb, 255:red, 14; green, 20; blue, 233 }] (734.64,88.71) .. controls (734.64,86.82) and (736.18,85.29) .. (738.07,85.29) .. controls (739.96,85.29) and (741.5,86.82) .. (741.5,88.71) .. controls (741.5,90.61) and (739.96,92.14) .. (738.07,92.14) .. controls (736.18,92.14) and (734.64,90.61) .. (734.64,88.71) -- cycle ;
%Shape: Circle [id:dp35655519493499854] 
\draw  [color={rgb, 255:red, 14; green, 20; blue, 233 }][fill={rgb, 255:red, 14; green, 20; blue, 233 }] (414.64,89.21) .. controls (414.64,87.32) and (416.18,85.79) .. (418.07,85.79) .. controls (419.96,85.79) and (421.5,87.32) .. (421.5,89.21) .. controls (421.5,91.11) and (419.96,92.64) .. (418.07,92.64) .. controls (416.18,92.64) and (414.64,91.11) .. (414.64,89.21) -- cycle ;
%Shape: Circle [id:dp19963716150832334] 
\draw  [color={rgb, 255:red, 14; green, 20; blue, 233 }][fill={rgb, 255:red, 14; green, 20; blue, 233 }] (276.64,88.71) .. controls (276.64,86.82) and (278.18,85.29) .. (280.07,85.29) .. controls (281.96,85.29) and (283.5,86.82) .. (283.5,88.71) .. controls (283.5,90.61) and (281.96,92.14) .. (280.07,92.14) .. controls (278.18,92.14) and (276.64,90.61) .. (276.64,88.71) -- cycle ;
%Straight Lines [id:da9527007126361247] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }]   (552.08,28.67) -- (552.08,48.84) ;
%Straight Lines [id:da8860441686225711] 
\draw [color={rgb, 255:red, 14; green, 20; blue, 233 }]   (571.17,78.67) -- (571.17,98.84) ;
%Straight Lines [id:da926646349979383] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }]   (742.17,28.51) -- (742.17,48.67) ;
%Straight Lines [id:da9830082600475529] 
\draw [color={rgb, 255:red, 14; green, 20; blue, 233 }]   (781.17,78.92) -- (781.17,99.09);
%Straight Lines [id:da7930422861136808] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }]   (552.08,38.76) -- (742.17,38.59);
%Straight Lines [id:da5196822535567758] 
\draw [color={rgb, 255:red, 14; green, 20; blue, 233 }]   (571.17,88.76) -- (781.17,89.01);

%Straight Lines [id:da8608373638765862] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }][line width=1] [dash pattern={on 3.75pt off 3.75pt}]  (513,4.89) -- (513,139.22) ;



% Text Node
\draw (18,25) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }] {T$_{1}$};

\draw (50,10) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }] {\Access$_{1}(X)$};

\draw (155,10) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }] {\Access$_{1}(Y)$};

\draw (240,22) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }] {\TryC{}$_{1}$};


% Text Node
\draw (212.43,78) node [anchor=north west] 
[color={rgb, 255:red, 14; green, 20; blue, 233 }] {T$_{2}$}; 

\draw (255.86,62) node [anchor=north west] 
[color={rgb, 255:red, 14; green, 20; blue, 233 }] {\Access$_{2}(X)$}; 

\draw (363.29,62) node [anchor=north west] 
[color={rgb, 255:red, 14; green, 20; blue, 233 }] {\Access$_{2}(Z)$}; 

\draw (460,75) node [anchor=north west] 
[color={rgb, 255:red, 40; green, 67; blue, 248 }] {\TryC{}$_{2}$};

\draw [color = {rgb, 255:red, 208; green, 2; blue, 27}] [fill  = {rgb, 255:red, 208; green, 2; blue, 27}] (120,130) -- (130,130) -- (130,140) -- (120,140) -- cycle;
\draw (129,121) node [anchor=north west] {(a) \rwOblivious{} model};



% Text Node
\draw (520,25) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128}] {T$_{1}$};

\draw (522,-8) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }, font = \small] {\Rset$_{1} = \{X\}$ \Wset$_{1} = \{Y\}$};

\draw (556,10) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }] {\Read$_{1}(X)$};

\draw (640,10) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }] {\Write$_{1}(Y,\ 10)$};

\draw (745,22) node [anchor=north west] 
[color={rgb, 255:red, 128; green, 128; blue, 128 }] {\TryC{}$_{1}$};


% Text Node
\draw (536,79) node [anchor=north west] 
[color={rgb, 255:red, 14; green, 20; blue, 233 }] {T$_{2}$};

\draw (538,100) node [anchor=north west] 
[color={rgb, 255:red, 14; green, 20; blue, 233}, font = \small] {\Rset$_{2} = \{X\}$ \Wset$_{2} = \{Z\}$};

\draw (579,62) node [anchor=north west] 
[color={rgb, 255:red, 14; green, 20; blue, 233 }] {\Read$_{2}(X)$};

\draw (680,62) node [anchor=north west] 
[color={rgb, 255:red, 14; green, 20; blue, 233 }] {\Write$_{2}(Z,\ 5)$};

\draw (780,75) node [anchor=north west] 
[color={rgb, 255:red, 40; green, 67; blue, 248 }] {\TryC{}$_{2}$};


\draw [color = {rgb, 255:red, 208; green, 2; blue, 27}] [fill  = {rgb, 255:red, 208; green, 2; blue, 27}] (540,130) -- (550,130) -- (550,140) -- (540,140) -- cycle;
\draw (548,121) node [anchor=north west] {(b) \rwAware{} model};


\end{tikzpicture}




